Clinical Utility of the Automatic Phenotype Annotation in Unstructured Clinical Notes: ICU Use Cases

Objective: Clinical notes contain information not present elsewhere, including drug response and symptoms, all of which are highly important when predicting key outcomes in acute care patients. We propose the automatic annotation of phenotypes from clinical notes as a method to capture essential information, which is complementary to typically used vital signs and laboratory test results, to predict outcomes in the Intensive Care Unit (ICU). Methods: We develop a novel phenotype annotation model to annotate phenotypic features of patients which are then used as input features of predictive models to predict ICU patient outcomes. We demonstrate and validate our approach conducting experiments on three ICU prediction tasks including in-hospital mortality, physiological decompensation and length of stay for over 24,000 patients by using MIMIC-III dataset. Results: The predictive models incorporating phenotypic information achieve 0.845 (AUC-ROC) to predict in-hospital mortality, 0.839 (AUC-ROC) for physiological decompensation and 0.430 (Kappa) for length of stay, all of which consistently outperform the baseline models leveraging only vital signs and laboratory test results. Moreover, we conduct a thorough interpretability study, showing that phenotypes provide valuable insights at the patient and cohort levels. Conclusion: The proposed approach demonstrates phenotypic information complements traditionally used vital signs and laboratory test results, improving significantly forecast of outcomes in the ICU.

==> tables/results_core_decomp_test_set.tex <==
\begin{table}[!htbp]
\centering
\scalebox{0.8}{
\begin{tabular}{|c|c|c|c|c|c|c|c|}
\hline
\multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}ML \\ Classification \\ Model\end{tabular}} & \multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}Features \\ Design\end{tabular}} & \multicolumn{4}{c|}{4-Fold Cross Validation Aggregate}     & \multicolumn{2}{c|}{Test Set}                                       \\ \cline{3-8} 
                                                                                       &                                                                             & \multicolumn{2}{c|}{AUC-ROC} & \multicolumn{2}{c|}{AUC-PR} & \multirow{2}{*}{AUC-ROC}         & \multirow{2}{*}{AUC-PR}          \\ \cline{3-6}
                                                                                       &                                                                             & Mean              & SD       & Mean              & SD      &                                  &                                  \\ \hline
\multirow{4}{*}{\begin{tabular}[c]{@{}c@{}}Random \\ Forest\end{tabular}}              & S                                                                           & 0.815            & 0.003   & \textbf{0.127}   & 0.009  & 0.826 (0.821, 0.831)          & \textbf{0.130 (0.123, 0.138)} \\ \cline{2-8} 
                                                                                       & S + NCR                                                                     & 0.820            & 0.003   & 0.124            & 0.007  & 0.825 (0.821, 0.830)          & 0.124 (0.118, 0.131)          \\ \cline{2-8} 
                                                                                       & S + CB                                                                      & 0.818            & 0.004   & 0.122            & 0.008  & 0.826 (0.821, 0.830)          & 0.125 (0.118, 0.132)          \\ \cline{2-8} 
                                                                                       & S + Ours                                                                    & \textbf{0.824}   & 0.002   & 0.125            & 0.006  & \textbf{0.827 (0.823, 0.832)} & 0.126 (0.119, 0.134)          \\ \hline
\multirow{4}{*}{\begin{tabular}[c]{@{}c@{}}Gradient \\ Boosting\end{tabular}}          & S                                                                           & 0.812            & 0.004  &\textbf{ 0.134}   & 0.010 & 0.830 (0.825, 0.835)          & 0.154 (0.146, 0.163)          \\ \cline{2-8}
                                                                                       & S + NCR                                                                     & 0.817            & 0.001  & 0.126            & 0.018 & 0.831 (0.827, 0.836)          & 0.124 (0.118, 0.131)          \\ \cline{2-8}
                                                                                       & S + CB                                                                      & 0.816            & 0.004   & 0.122            & 0.023  & 0.834 (0.829, 0.838)          & 0.157 (0.149, 0.165)          \\ \cline{2-8}
                                                                                       & S + Ours                                                                     & \textbf{0.823}   & 0.005  & 0.131            & 0.014  &\textbf{ 0.838 (0.833, 0.842)} & \textbf{0.162 (0.154, 0.171)} \\ \hline
\multirow{5}{*}{LSTM}                                                                  & \begin{tabular}[c]{@{}c@{}}S \cite{harutyunyan2019multitask}\end{tabular}   & -                 & -        & -                 & -       & 0.809                            & 0.125                           \\ \cline{2-8} 
                                                                                       & S                                                                           & 0.819            & 0.002   & 0.135            & 0.016  & 0.824 (0.819, 0.829)          & 0.126 (0.119, 0.133)          \\ \cline{2-8} 
                                                                                       & S + NCR                                                                     & 0.820            & 0.003   & 0.133            & 0.012  & 0.834 (0.829, 0.839)          & 0.134 (0.127, 0.142)          \\ \cline{2-8} 
                                                                                       & S + CB                                                                      & 0.820            & 0.005   & 0.128            & 0.021  & 0.833 (0.828, 0.838)          & 0.114 (0.108, 0.119)          \\ \cline{2-8} 
                                                                                       & S + Ours                                                                    & \textbf{0.833}   & 0.007   & \textbf{0.144}   & 0.022  & \textbf{0.839 (0.834, 0.844)} & \textbf{0.145 (0.138, 0.153)} \\ \hline
\end{tabular}}
\caption{ICU Decompensation Results with Area Under the Curve of Receiver Operating Characteristic (AUC-ROC) and Area Under the Curve of Precision-Recall (AUC-PR) Scores. Test set scores are shown with 95\% confidence intervals. The best score for each classifier is highlighted in bold. Here, S refers to Structured, NCR to Neural Concept Recognizer\cite{arbabi2019ncr}, CB to ClinicalBERT, and Ours to our phenotyping model.}
\label{table:results_core_decomp}
\end{table}

==> tables/results_core_los_test_set.tex <==
\begin{table}[!htbp]
\centering
\scalebox{0.8}{
\begin{tabular}{|c|c|c|c|c|c|c|c|}
\hline
\multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}ML \\ Classification \\ Model\end{tabular}} & \multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}Features \\ Design\end{tabular}} & \multicolumn{4}{c|}{4-Fold Cross Validation Aggregate}   & \multicolumn{2}{c|}{Test Set}                                             \\ \cline{3-8} 
                                                                                       &                                                                             & \multicolumn{2}{c|}{Kappa} & \multicolumn{2}{c|}{MAD}    & \multirow{2}{*}{Kappa}           & \multirow{2}{*}{MAD}                   \\ \cline{3-6}
                                                                                       &                                                                             & Mean             & SD      & Mean              & SD      &                                  &                                        \\ \hline
\multirow{4}{*}{\begin{tabular}[c]{@{}c@{}}Random \\ Forest\end{tabular}}              & S                                                                           & 0.381           & 0.004  & \textbf{142.0} & 4.6  & 0.390 (0.388, 0.392)          & \textbf{136.8 (136.2, 137.4)} \\ \cline{2-8} 
                                                                                       & S + NCR                                                                     & 0.382           & 0.007  & 148.0          & 4.1  & 0.390 (0.388, 0.392)          & 142.5 (141.9, 143.1)          \\ \cline{2-8} 
                                                                                       & S + CB                                                                      & 0.369           & 0.005  & 149.2          & 3.7  & 0.376 (0.374, 0.379)          & 144.3 (143.7, 144.9)          \\ \cline{2-8} 
                                                                                       & S + Ours                                                                    & \textbf{0.395}  & 0.006  & 146.2          & 4.6  & \textbf{0.405 (0.403, 0.407)} & 140.6 (140.0, 141.2)          \\ \hline
\multirow{4}{*}{\begin{tabular}[c]{@{}c@{}}Gradient \\ Boosting\end{tabular}}          & S                                                                           & 0.387           & 0.001  & 155.9          & 2.1  & 0.399 (0.397, 0.401)          & 151.8 (151.1, 152.4)              \\ \cline{2-8} 
                                                                                       & S + NCR                                                                     & 0.366           & 0.005  & 150.2          & 3.0  & 0.381 (0.378, 0.383)          & 146.7 (146.1, 147.3)          \\ \cline{2-8} 
                                                                                       & S + CB                                                                      & 0.373           & 0.005  & 148.8          & 2.7  & 0.392 (0.390, 0.394)          & 143.5 (143.0, 144.1)            \\ \cline{2-8} 
                                                                                       & S + Ours                                                                    & \textbf{0.401}  & 0.003  & \textbf{142.0} & 3.7  & \textbf{0.412 (0.410, 0.414)} & \textbf{138.9 (138.3, 139.5)}   \\ \hline
\multirow{5}{*}{LSTM}                                                                  & S \cite{harutyunyan2019multitask}                                           &                  &         &                   &         & 0.395                           & 126.7                               \\ \cline{2-8} 
                                                                                       & S                                                                           & 0.375           & 0.003  & 134.3          & 17.2 & 0.380 (0.377, 0.382)          & 157.0 (156.3, 157.6)          \\ \cline{2-8} 
                                                                                       & S + NCR                                                                     & 0.392           & 0.013  & 127.1          & 17.4 & 0.406 (0.404, 0.408)          & 123.3 (122.8, 123.9)          \\ \cline{2-8} 
                                                                                       & S + CB                                                                      & 0.374           & 0.015  & 127.6          & 8.6  & 0.388 (0.386, 0.390)          & 120.1 (119.6, 120.6)          \\ \cline{2-8} 
                                                                                       & S + Ours                                                                    & \textbf{0.416}  & 0.011  & \textbf{116.1} & 6.9  & \textbf{0.430 (0.427, 0.432)} & \textbf{116.7 (116.1, 117.2)} \\ \hline
\end{tabular}}
\caption{ICU Length of Stay Results with Cohen's Kappa and Mean Absolute Deviation (MAD) Scores. Test set scores are shown with 95\% confidence intervals. The best score for each classifier is highlighted in bold. Here, S refers to Structured, NCR to Neural Concept Recognizer\cite{arbabi2019ncr}, CB to ClinicalBERT, and Ours to our phenotyping model.}
\label{table:results_core_los}
\end{table}

==> tables/results_core_mortality_test_set.tex <==
\begin{table}[!htbp]
\centering
\scalebox{0.80}{
\begin{tabular}{|c|c|c|c|c|c|c|c|}
\hline
\multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}ML \\ Classification \\ Model\end{tabular}} & \multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}Features \\ Design\end{tabular}} & \multicolumn{4}{c|}{4-Fold Cross Validation Aggregate}     & \multicolumn{2}{c|}{Test Set}                                       \\ \cline{3-8} 
                                                                                       &                                                                             & \multicolumn{2}{c|}{AUC-ROC} & \multicolumn{2}{c|}{AUC-PR} & \multirow{2}{*}{AUC-ROC}         & \multirow{2}{*}{AUC-PR}          \\ \cline{3-6}
                                                                                       &                                                                             & Mean              & SD       & Mean              & SD      &                                  &                                  \\ \hline
SAPS-II                                                                                & -                                                                           & 0.754            & 0.006   & 0.322            & 0.031  & 0.756                           & 0.312                           \\ \hline
APACHE-III                                                                             & -                                                                           & 0.732            & 0.008   & 0.326            & 0.018  & 0.733                           & 0.308                           \\ \hline
\multirow{4}{*}{\begin{tabular}[c]{@{}c@{}}Random \\ Forest\end{tabular}}              & S                                                                           & 0.809            & 0.008   & 0.417            & 0.018  & 0.800 (0.775, 0.824)          & 0.339 (0.286, 0.395)          \\ \cline{2-8} 
                                                                                       & S + NCR                                                                     & 0.818            & 0.014   & \textbf{0.472}   & 0.013  & 0.828 (0.802, 0.853)          & \textbf{0.467 (0.404, 0.529)} \\ \cline{2-8} 
                                                                                       & S + CB                                                                      & 0.803            & 0.011   & 0.423            & 0.004  & 0.812 (0.787, 0.838)          & 0.403 (0.345, 0.463)          \\ \cline{2-8} 
                                                                                       & S + Ours                                                                     & \textbf{0.829}   & 0.008   & 0.458   & 0.017  & \textbf{0.833 (0.809, 0.857)} & 0.396 (0.340, 0.456) \\ \hline
\multirow{5}{*}{LSTM}                                                                  & S \cite{harutyunyan2019multitask}                                           & -                 & -        & -                 & -       & 0.825                           & 0.410                           \\ \cline{2-8} 
                                                                                       & S                                                                           & 0.828           & 0.007  & 0.441           & 0.015 & 0.826 (0.801, 0.848)          & 0.391 (0.334, 0.452)          \\ \cline{2-8} 
                                                                                       & S + NCR                                                                     & 0.835           & 0.010  & 0.478           & 0.008 & 0.841 (0.818, 0.864)          & 0.453 (0.393, 0.513)          \\ \cline{2-8} 
                                                                                       & S + CB                                                                      & 0.828           & 0.007  & 0.459           & 0.006 & 0.826 (0.802, 0.849)          & 0.414 (0.355, 0.476)          \\ \cline{2-8} 
                                                                                       & S + Ours                                                                     & \textbf{0.844}  & 0.004  & \textbf{0.495}  & 0.013 & \textbf{0.845 (0.823, 0.868)} & \textbf{0.464 (0.405, 0.523)} \\ \hline
\end{tabular}}
\caption{ICU In-Hospital Mortality Results with Area Under the Curve of Receiver Operating Characteristic (AUC-ROC) and Area Under the Curve of Precision-Recall (AUC-PR) Scores. Test set scores are shown with 95\% confidence intervals. The best score for each classifier is highlighted in bold. Here, S refers to Structured, NCR to Neural Concept Recognizer\cite{arbabi2019ncr}, CB to ClinicalBERT, and Ours to our phenotyping model.}
\label{table:results_core_mortality}
\end{table}
